Essential twisted surfaces in alternating link complements

Checkerboard surfaces in alternating link complements are used frequently to determine information about the link. However, when many crossings are added to a single twist region of a link diagram, the geometry of the link complement stabilizes (approaches a geometric limit), but a corresponding checkerboard surface increases in complexity with crossing number. In this paper, we generalize checkerboard surfaces to certain immersed surfaces, called twisted checkerboard surfaces, whose geometry better reflects that of the alternating link in many cases. We describe the surfaces, show that they are essential in the complement of an alternating link, and discuss their properties, including an analysis of homotopy classes of arcs on the surfaces in the link complement.

==> trisquares-twc03614-arxiv.tex <==
%% The explanation below should probably go into section 4:
%%
%% To simplify notation, we will refer to an edge and its image in the
%% diagram of $L_{B,i}$ by the same letter.  Thus $f$ is simultaneously
%% the edge in Figure \ref{fig:tri-squares-labels} and a curve in the
%% diagram of $L_{B,i}$.  

The main result of this section is that the graph $\Gamma_B$ of Lemma~\ref{lemma:graph-bluevalence} cannot contain three and five adjacent bigons, for $L_{B,0}$ and $L_{B,2}$, respectively.  To prove this, we examine adjacent triangles and squares.

Suppose a blue--blue--red triangle in $\Gamma_{BR}$ is adjacent to a blue and red square, adjacent across the red edge, as illustrated on the left of Figure~\ref{fig:tri-squares-labels}.  We will call this a \emph{triangle--square pair}.  In this section, we examine adjacent triangle--square pairs, adjacent at the vertex of the triangle.  We show that in $L_{B,0}$ there cannot be three adjacent triangle--square pairs, and in $L_{B,2}$ there cannot be five adjacent triangle--square pairs.

\begin{figure}
  \includegraphics{trisquare-pair} \hspace{.5in}
  \input{trisquare-labels.pspdftex}
  \caption{Left: A triangle--square pair.  Right: Three adjacent
    triangle--square pairs will be labeled as shown.}
  \label{fig:tri-squares-labels}
\end{figure}

Label three adjacent triangles and squares as in Figure~\ref{fig:tri-squares-labels}.  By Lemma~\ref{lemma:distinct-crossings}, each triangle shown meets distinct crossings.  Thus the diagram may have two, three, or four crossings coming from the intersections of blue and red edges of triangles.  Up to symmetry, there are exactly four possibilities, shown in Figure~\ref{fig:trisquare-options}.

\begin{figure}
  \input{threeadjoptions.pspdftex}
  \caption{Possibilities for three adjacent triangles.}
  \label{fig:trisquare-options}
\end{figure}

Note the diagrams shown are only sketches.  In options I and II, the curve $i \cup j$ must run through the crossing disk, and in option III, the curve $i\cup j\cup k$ must run through the crossing disk.  We have chosen to show $j$ running through the disk in I and II, and $k$ in III.  Additionally, we have chosen to show none of $i$, $j$, or $k$ running through the crossing disk in option IV.  However, a priori, these are arbitrary choices.  Hence we must be careful to ensure that our arguments below do not depend on these choices.
%% or that we may isotope the diagram to ensure the crossing disk actually intersects the red edges as shown.

For all four possibilities, we have the following lemma.

\begin{lemma}\label{lemma:fg-endpoints}
Suppose the edge labeled $f$ in Figure \ref{fig:tri-squares-labels} is not mapped into the region of the diagram of $K_{B,i}$ containing images of edges labeled $a$ and $c$.  Then $f$ cannot have both of its endpoints mapped to the same crossing of $K_{B,i}$.  Similarly, if $g$ is not mapped into the same region as edges labeled $b$ and $d$, then $g$ cannot have both of its endpoints mapped to the same crossing.
\end{lemma}

\begin{proof}
We will prove the lemma for $f$.  The argument for $g$ is symmetric.  Again we will refer to an edge in Figure~\ref{fig:tri-squares-labels} and its image in the diagram of $L_{B,i}$ by the same name.

Suppose $f$ is not in the region of $a$ and $c$, but $f$ has both endpoints on the same crossing.  Then $f$ forms a loop in a blue region.
By our assumption that complexity is minimal, $f$ cannot be homotoped away from this blue region.  Thus it meets a crossing disk $G$.  Note that since $f$ does not meet the region of $a$ and $c$ by assumption, and $f$ cannot meet the region of $b$ by Lemma~\ref{lemma:blue-prime}\eqref{lmitm:distinct-regions-cross}, $G$ is disjoint from the crossing disk corresponding to the vertex at $a$, $b$, $c$ and $d$.

First, we claim that $G$ meets the edge $i$.  Because $f$ intersects $G$, there are green edges $\gamma_1$ and $\gamma_2$, each with one endpoint on $f$, running through squares $eif\ell$ and $fjgm$ of Figure~\ref{fig:tri-squares-labels}, respectively, corresponding to intersections with $G$.  If $\gamma_1$ meets $i$, then the claim is proved.  So suppose $\gamma_1$ meets $e$ or $\ell$.  By Lemma~\ref{lemma:no-green-meets-bcj}, $\gamma_2$ cannot meet $j$, so $\gamma_2$ meets either $m$ or $g$.  Finally, Lemma~\ref{lemma:RGB-adjacent-blue} implies that we cannot simultaneously have $\gamma_1$ meeting $\ell$ and $\gamma_2$ meeting $m$.  Thus either $\gamma_1$ meets $e$ or $\gamma_2$ meets $g$.  After mapping to the diagram, endpoints of $e$ and $g$ are separated from those of $f$ by the closed curve $a \cup c \cup i \cup j$.  Note that Lemma~\ref{lemma:blue-prime}\eqref{lmitm:distinct-regions-cross} implies $e$ cannot meet the region of $a$ (which is also the region of $c$), and $g$ cannot meet the region of $c$ (also the region of $a$).  Hence the only way for $\gamma_1$ to meet $e$ or $\gamma_2$ to meet $g$ is if $G$ runs over $i$ or $j$.  It does not meet $j$ by Lemma~\ref{lemma:no-green-meets-bcj}.  Hence $G$ meets $i$, as claimed.

Now, $G$ intersects $i$, so a green edge lies in the triangle $abi$. By Lemma~\ref{lemma:no-green-meets-bcj}, it does not run to $b$.  Thus it runs from $i$ to $a$.  Since $f$ and $a$ are in distinct regions, by assumption, $a$ and $f$ must meet this green disk on opposite sides, as in Figure~\ref{fig:af-oppsides}.

\begin{figure}
  \input{afi-intgreen.pspdftex}
  %% \includegraphics{figures/af-oppsides.pdf}
  \caption{Edges $a$, $f$, and $i$ intersect some green crossing disk}
  \label{fig:af-oppsides}
\end{figure}

Now, edges $e$ and $\ell$ meet at a crossing.  The edge $e$ cannot be in the region of $a$ by Lemma~\ref{lemma:blue-prime}\eqref{lmitm:distinct-regions-cross}.
The edge $e$ cannot lie in the region containing $f$ because these are separated by $a \cup i\cup j \cup c$.  So $e$ cannot meet $G$.
Therefore, the only way for $\ell$ to meet the endpoint of $e$ is for $\ell$ to run through $G$.  Hence a green edge runs through the square $eif\ell$ with one endpoint on $\ell$.  That edge cannot meet $i$, by Lemma~\ref{lemma:red-green-bigons}.  It cannot meet $e$ because $e$ is disjoint from $G$.  So it meets $f$ and continues into a green edge in the square $fmgj$.  This green edge cannot meet $j$, by Lemma~\ref{lemma:no-green-meets-bcj}.  It cannot meet $m$ by Lemma~\ref{lemma:RGB-adjacent-blue}.  It cannot meet $g$, or $a$ and $g$,
therefore $c$ and $g$, are in the same region, contradicting Lemma~\ref{lemma:blue-prime}\eqref{lmitm:distinct-regions-cross}. This gives a
contradiction.
\end{proof}

\begin{lemma}\label{lemma:fg-regions}
If the edge labeled $f$ in Figure~\ref{fig:tri-squares-labels} is mapped to the same region as edges labeled $a$ and $c$, then the crossing at the endpoints of images of $b$ and $f$ is associated to the crossing circle corresponding to the common vertex of the triangles of Figure~\ref{fig:tri-squares-labels}, and in addition, at least one of the crossings at the endpoints of images of $h$ and $d$ or of $g$ and $c$ is associated to the same crossing circle.
\end{lemma}

Notice that Lemma~\ref{lemma:fg-regions} implies something symmetric for $g$ by flipping the adjacent triangle--square pairs upside down and relabeling: If $g$ is mapped to the region of images of $b$ and $d$, then the crossing at the endpoints of images of $c$ and $g$ is associated to the crossing circle of the vertex, in addition to at least one of the crossings at the endpoints of images of $e$ and $a$ or $b$ and $f$.

\begin{proof}
Again we refer to edges and their images by the same name.  Suppose that $f$ is in the region of $a$ and $c$.  Then Lemma~\ref{lemma:blue-prime}\eqref{lmitm:assoc-cross} implies that the crossing meeting endpoints of $f$ and $b$ is associated with the crossing circle $C$ corresponding to the vertex of the graph.

Suppose that the crossing at the endpoints of $d$ and $h$ is not associated to $C$.  This implies that $h$ cannot be in the region of $a$ and $c$, by Lemma~\ref{lemma:blue-prime}\eqref{lmitm:assoc-cross}.  In cases I and III of Figure~\ref{fig:trisquare-options}, $h$ is automatically either in the region of $f$ or in the region of $a$ and $c$, so these cases are impossible.  Thus we are either in case II or IV.

Notice that there are two versions of case II, where the crossings at the ends of $a$ and $c$ are the same, and where the crossings at the ends of $b$ and $d$ are the same.  In the latter case, we deduce that the crossing at the endpoints of $d$ and $h$ must be associated with $C$.  So we may assume in case II that the crossings at the ends of $a$ and $c$ are the same, as shown in Figure~\ref{fig:trisquare-options}.  

Now suppose that the crossing at the endpoints of $c$ and $g$ is not associated to the crossing circle.  Then $g$ cannot meet the region of $b$ and $d$ by Lemma~\ref{lemma:blue-prime}\eqref{lmitm:assoc-cross}.  By Lemma~\ref{lemma:fg-endpoints} it cannot have both endpoints on the same crossing.  But the endpoint of $g$ is contained in the region bounded by $b \cup j \cup k \cup d$.  Thus the other endpoint of $g$ must also be contained in that region, and must lie on a new crossing disjoint from the existing crossings in the diagram, as in Figure~\ref{fig:g-newcrossing}.

\begin{figure}
  \input{gdistinctcrossing.pspdftex}
  %% \includegraphics{figures/g-newcrossing.pdf}
  \caption{Edge $g$ meets a new crossing within the region bounded by $b\cup j\cup k
    \cup d$}
  \label{fig:g-newcrossing}
\end{figure}

Edges $n$ and $h$ have endpoints on the same crossing, but their other endpoints are bounded away from each other by $b\cup j\cup k\cup d$.  Because $h$ does not meet the region of $b$ or $d$, the edge $n$ must either meet $k$ or $j$.

Suppose first that $n$ meets $j$.  Then $n$ crosses into a region bounded away from the endpoint of $h$ by $a \cup c \cup i \cup j$.
We may assume, by applying a small homotopy which does not change the graphs $\Gamma_B$, $\Gamma_{BR}$, and $\Gamma_{BRG}$, that $n$ intersects $j$ at most once.  
Since $h$ does not meet the region of $a$ or $c$, the edge $n$ must then run through $i$.  But then $f$ is separated from the region of $a$ and $c$ by red edges, contradicting assumption.

So we conclude that $n$ meets the edge $k$.  Now, the edge $g$ along with a portion of $n$ and a portion of $k$ form a closed curve $\gamma$ meeting the diagram of $K_{B,i}$ twice with crossings on either side. Lemma~\ref{lemma:K2-0-prime} implies that we are in the diagram of $K_{B,0}$, and one of the red arcs, either $n$ or $k$, must meet a green disk.  Moreover, the closed curve $\gamma$ intersects this green disk transversely, exactly once.

Suppose first that $k$ meets a green disk $G$.  Then there is a green edge inside the triangle $cdk$, which must run from $k$ to $d$ by Lemma~\ref{lemma:no-green-meets-bcj}, hence $d$ also meets $G$.
Since the portions of $k \cup n$ making up $\gamma$ intersect $G$ only once, the diagram must be as in Figure~\ref{fig:n-meets-k-1}, left. (Note that $d$ cannot cross $g$ since they are in distinct regions.) Now consider the portion of $d$ shown in that figure, along with a portion of $k$ and an arc on $G$.  This forms a new closed curve $\gamma'$ meeting the diagram exactly twice, with crossings on either side.  If the portion of $\gamma'$ on the red meets another green disk, again the disk must meet $d$, so we may replace $\gamma'$ by a smaller closed curve consisting of an arc on the new green disk, and remnants of $\gamma'$, as in the proof of Lemma~\ref{lemma:red-blue-bigons}.  As in the proof of that lemma, by induction, we obtain a simple closed curve meeting the diagram of $K_{B,0}$ twice without meeting any crossing disks, and with crossings on both sides, contradicting Lemma~\ref{lemma:K2-0-prime}.

\begin{figure}
  \input{nmeetsk.pspdftex}
  %% \includegraphics{figures/n-meets-k.pdf}
  \caption{Left:  Crossing disk meeting $k$ and $d$.  Right:  Crossing
  disk meeting $n$ and $g$.}
  \label{fig:n-meets-k-1}
\end{figure}

Hence $n$ must meet a crossing disk $G$ between the endpoint of $n$ at $g$ and the point where $n$ meets $k$.  Thus there is a green edge with endpoint on $n$ in the square $gnhk$.  This edge cannot have its other endpoint on $k$, by Lemma~\ref{lemma:red-green-bigons}.  We claim it cannot have an endpoint on $h$.  This is because $h$ has both endpoints in the region bounded by $b\cup j\cup k\cup d$.  If the green edge happened to end on $h$, then the green disk must cross $b \cup j \cup k \cup d$.  It cannot cross $j$, by Lemma~\ref{lemma:no-green-meets-bcj}.  If it crosses $b$ or $d$, then either $g$ or $h$ must be in the region of $b$ and $d$, which is impossible by assumption, and by Lemma~\ref{lemma:blue-prime}\eqref{lmitm:distinct-regions-cross}.  If $G$ meets $k$, then there is a green arc in the triangle $cdk$, which again implies $G$ meets $d$, and so $g$ or $h$ is in the region of $b$ and $d$, which is impossible.  

Thus the green edge in square $gnhk$ with one endpoint on $n$ has its other endpoint on $g$.  Because the portion of $n \cup k$ making up $\gamma$ meets the crossing disk exactly once, the disk must be as shown in Figure~\ref{fig:n-meets-k-1}, right.  Again portions of $n$, $g$, and the crossing disk form a simple closed curve $\gamma'$ meeting the diagram of $K_{B,0}$ exactly twice.  Again, as in the proof of Lemma~\ref{lemma:red-blue-bigons}, replacing this closed curve if necessary, we obtain a contradiction to Lemma~\ref{lemma:K2-0-prime}.
\end{proof}

\begin{lemma}\label{lemma:tri-squares-assoc}
If there are three adjacent triangle--square pairs, as in Figure
\ref{fig:tri-squares-labels}, then for one of the following pairs of
crossings, both crossings are associated to the crossing circle
corresponding to the vertex:
\begin{enumerate}
\item crossings at the endpoints of $f$ and $b$ and of $d$ and $h$, or
\item crossings at the endpoints of $f$ and $b$ and of $g$ and $c$, or 
\item crossings at the endpoints of $g$ and $c$ and of $a$ and $e$.
\end{enumerate}
\end{lemma}

\begin{proof}
We prove the lemma by contradiction.  By Lemmas \ref{lemma:fg-regions} and \ref{lemma:fg-endpoints}, if there are three adjacent triangles and squares but the result does not hold, then edges $f$ and $g$ cannot be in the regions of edges $a$ and $c$, and $b$ and $d$, respectively, and neither $f$ nor $g$ can have endpoints on the same crossing.  Thus $f$ ends in a new crossing in the region $a \cup i \cup j \cup c$, and $g$ ends in a new crossing in the region $b \cup d \cup j \cup k$.

We may add these new crossings to Figure \ref{fig:trisquare-options}. However, first note that in options I and II from that figure, we have sketched the diagram so that $j$ runs through the crossing disk corresponding to the vertex of the graph.  In fact, if $j$ runs through that crossing disk, then a green edge corresponding to this crossing disk runs through the square $fmgj$, with one endpoint on $j$.  By Lemma \ref{lemma:red-green-bigons}, the other endpoint must be either on $f$ or $g$.  This implies that either $f$ meets the region of $a$ and $c$, or $g$ meets the region of $b$ and $d$, both of which we have ruled out.  Hence we need to adjust the diagrams of I and II so that $i$ meets the crossing disk corresponding to the vertex instead of $j$.  In III and IV, $i$ or $k$ might meet that crossing disk as well, but the same argument shows that $j$ cannot.  Updated sketches of the four possibilities are shown in Figure \ref{fig:fg-terminate}.

\begin{figure}
  \input{3adjupdate.pspdftex}
  %% \includegraphics[width=5in]{figures/fg-terminate.pdf}
  \caption{Four possibilities for endpoints of $f$ and $g$}
  \label{fig:fg-terminate}
\end{figure}

Note that the two endpoints of $m$ are shown in each figure.  In order for these endpoints to join, either $m$ must intersect $j$, or the crossing disk corresponding to the vertex.  This is because the endpoints of $m$ are separated by the closed curve $b \cup j \cup c \cup (\mbox{crossing disk})$.

Suppose first that $m$ intersects $j$.  Then $f$, along with a portion of $j$ and a portion of $m$, form a closed curve meeting the diagram of $K_{B,i}$ twice with crossings on either side.  Lemma~\ref{lemma:K2-0-prime} immediately implies that the diagram is that of $K_{B,0}$, not $K_{B,2}$.  Lemmas~\ref{lemma:K2-0-prime} and~\ref{lemma:no-green-meets-bcj} imply that the portion of $m$ meets some green crossing disk.  Then there is a green edge in the square $fmgj$ meeting either the edge $f$ or $g$. If $f$, then we may choose such a crossing disk closest to the crossing shared by $m$ and $f$, and argue as in the proof of the previous lemma that we obtain a contradiction to Lemma~\ref{lemma:K2-0-prime}.  So the green edge runs from $m$ to $g$.  But this green crossing disk must be contained in the region bounded by $i \cup j \cup a \cup c$, or have endpoints in the region of $a$ and $c$.  Since $g$ cannot meet the region of $a$ and $c$, we obtain a contradiction.

The only remaining possibility is that $m$ intersects the crossing disk corresponding to the vertex.  Then there is a corresponding green edge running through the square $fmgj$, with one endpoint on $m$.  Lemma~\ref{lemma:red-green-bigons} implies its other endpoint is not on $j$.  Hence its endpoint is on $f$ or $g$.  But that is possible only if $f$ is in the region of $a$ and $c$, or $g$ is in the region of $b$ and $d$.
\end{proof}


\begin{lemma}\label{lemma:No-fg-assoc}
If there are three adjacent triangle--square pairs as in Figure \ref{fig:tri-squares-labels}, then it cannot be the case that the crossings at the endpoints of images of $b$ and $f$ and of $c$ and $g$ are both simultaneously associated to the crossing circle corresponding to the vertex.
\end{lemma}

\begin{proof}
By Lemma~\ref{lemma:distinct-crossings}, the crossing at the endpoints of $f$ and $b$ and the crossing at the endpoints of $g$ and $c$ must be distinct.  Suppose both are associated to the crossing circle corresponding to the vertex, call it $C$. Then there are two distinct crossings associated to $C$, so the diagram cannot be that of $L_{B,0}$ by definition.  Hence we may assume that the diagram is that of $L_{B,2}$ and no additional crossings are associated to $C$.

Consider each of the options from Figure~\ref{fig:trisquare-options}.
We will show none of these can occur.

First consider option I.  The diagram has two crossings shown, and by assumption both of those crossings are associated to the crossing circle shown.  This means the region of $a$ and $c$ is the region of $f$ and $h$, and the region of $b$ and $d$ is the region of $e$ and $g$.  Then we can draw arcs in these regions from one crossing to another.  These arcs, along with the edges $i$ and $j$, will give closed curves in the diagram of $K_{B,2}$ meeting the diagram twice. Because the diagram of $K_{B,2}$ is prime, each bounds a strand of the knot and no crossings.  Thus the diagram of $K_{B,2}$ is that of a $(2,2)$--torus link, with a crossing circle of $L_{B,2}$ encircling the two crossings.  This contradicts Lemma~\ref{lemma:22torus}.

Now consider option II.  By assumption, the edge $f$ is in the region of $a$ and $c$, the edge $g$ is in the region of $b$ and $d$.  Draw an arc $\alpha$ inside the region of $b$ and $d$ from the crossing at the endpoint of $e$ (and $g$) to the crossing at the endpoint of $b$.  Now $\alpha \cup i$ meets the diagram of $K_{B,2}$ twice, with crossings on either side.  This contradicts Lemma \ref{lemma:K2-0-prime}.

For option III, note the crossing at endpoints of $a$ and $d$ must be associated to the crossing circle shown, by Lemma~\ref{lemma:blue-prime}\eqref{lmitm:assoc-cross}.  By assumption, the other two crossings are associated to that crossing circle as well. Thus three distinct crossings are associated to the crossing circle, contradicting the definition of $L_{B,2}$.

Finally, consider option IV.  Since the crossings at endpoints of $b$ and $f$ and of $c$ and $g$ are associated with the crossing circle shown, the crossing disk it bounds intersects the edge labeled $j$, by our convention on the diagram of Definition~\ref{def:L0-L2}.  Now consider the green edges of intersection in the graph.  One green edge runs from the vertex to $j$.  From there, a green edge must run to $f$ or $g$, but not $m$ by Lemma~\ref{lemma:red-green-bigons}.  The cases $f$ and $g$ are symmetric, so suppose it runs to $f$.  Now there must be a green edge in the square $eif\ell$.  It cannot run from $f$ to $i$, by Lemma \ref{lemma:RGB-adjacent-blue}.  It cannot run from $f$ to $e$, or $e$ would be in the region of $b$ and $d$, and Lemma~\ref{lemma:blue-prime}\eqref{lmitm:assoc-cross} would imply that a third crossing is associated to the crossing circle shown, which is a contradiction.  Thus the green edge runs from $f$ to $\ell$, and $\ell$ must be parallel to $j$ in the red bigon region containing $j$.  But then $e$ meets one of the crossings at the endpoints of $j$, either at the endpoint of $b$ or at the endpoint of $c$.  If $e$ meets $b$, then $e$ belongs to the region of $b$, and again we have too many crossings associated to the crossing circle.  If $e$ meets $c$, we get a contradiction to Lemma~\ref{lemma:blue-prime}\eqref{lmitm:distinct-regions}.
\end{proof}

\begin{lemma}\label{lemma:ae-assoc}
In three adjacent triangle--square pairs as in Figure~\ref{fig:tri-squares-labels}, if the crossings at the endpoints of $f$ and $b$ and of $h$ and $d$ are both associated to the crossing circle of the vertex, then so is the crossing at the endpoint of $a$ and $e$.
\end{lemma}

\begin{proof}
Suppose first that the crossings at the endpoints of $f$ and $b$ and at the endpoints of $h$ and $d$ are actually the same crossing.  If that crossing is associated to the crossing circle of the vertex, call it $C$, then Lemma~\ref{lemma:No-fg-assoc} implies that the crossing at the endpoints of $g$ and $c$ is not associated to $C$.  Assume by way of contradiction that the crossing at the endpoints of $a$ and $e$ is also not associated $C$.  Then Lemma~\ref{lemma:blue-prime}\eqref{lmitm:assoc-cross} implies that neither $g$ nor $e$ can meet a region meeting $C$, hence both $g$ and $e$ are disjoint from the crossing disk bounded by $C$.

Since $C$ is associated to the crossing at endpoints of $f$ and $b$, we know that the corresponding crossing disk intersects either $i$ or $j$, by our convention on diagrams (Definition~\ref{def:L0-L2}).  The arguments for both are nearly identical (in fact, symmetric in the squares $fjgm$ and $ief\ell$). We will walk through the argument for $j$ and leave the case of $i$ to the reader.  So suppose there is a green edge with one endpoint on $j$ running through the square $fjgm$.  The other endpoint cannot lie on $m$, by Lemma~\ref{lemma:red-green-bigons}.  It cannot lie on $g$ by our above observation that $g$ is disjoint from this crossing disk.  Hence the green edge runs from $j$ to $f$.  See Figure~\ref{fig:bd-sameassoc}.

\begin{figure}
  \input{bd-sameassoc.pspdftex}
  \caption{Left: Form of diagram if crossing at endpoints of $b$ and $d$ agree, and is associated to the crossing circle of the vertex.}
  \label{fig:bd-sameassoc}
\end{figure}

But then there is a green edge in the square $eif\ell$ with one endpoint on $f$.  It cannot have its other endpoint on $i$ by Lemma~\ref{lemma:RGB-adjacent-blue}.  It cannot have its other endpoint on $e$ since $e$ is disjoint from the region of $C$.  Thus its final endpoint is on $\ell$, and so $\ell$ runs through the crossing disk. But then $\ell$ has an endpoint on the crossing at endpoints of $b$, $j$, and $f$.  Because the square $eif\ell$ and the triangle $bcj$ are both mapped either above or below the projection plane (in Figure~\ref{fig:bd-sameassoc}, they are shown mapped below), Lemma~\ref{lemma:edge-intersections}\eqref{lmitm:blue-red} implies that $j$ and $b$ meet in the same regions of the diagram as $\ell$ and a blue edge meeting $\ell$ in a vertex.  So either $e$ or $f$ is the same region as $b$.  The edge $f$ cannot be in the region of $b$ by Lemma~\ref{lemma:blue-prime}\eqref{lmitm:distinct-regions-cross}.  But the edge $e$ cannot be in the region of $b$ either, because $e$ is not in a region meeting $C$.

This contradiction implies that if both the crossing at the endpoints of $f$ and $b$ and the crossing at the endpoints of $h$ and $d$ are associated with $C$, then they must be distinct crossings. So, the diagram cannot be that of $L_{B,0}$.

But now notice that if two crossings are associated to the same crossing circle, then they come from the same twist region, so there is a (red) bigon between them.  Then either $j$ lies in that bigon region or $i$ does.  If $j$ lies in the bigon, then its two endpoints must lie on the two crossings of the bigon.  Hence $c$ has an endpoint on one of those two crossings, and it is associated with the crossing circle of the vertex.  This contradicts Lemma \ref{lemma:No-fg-assoc}.  Thus $i$ lies in the bigon region between the two crossings.  It follows that $a$ has its endpoint on the crossing meeting $d$.  Thus the crossing at the endpoints of $a$ and $e$ is the same as the crossing at the endpoint of $d$ and $h$, and so it must be associated to the crossing circle corresponding to the vertex.  
\end{proof}


\begin{lemma}\label{lemma:L0-no-3trisquares}
There cannot be three adjacent triangle--square pairs for the diagram of $L_{B,0}$.  
\end{lemma}

\begin{proof}
Lemma \ref{lemma:tri-squares-assoc} implies that images of edges from the triangle--square pairs must meet at two crossings associated to the crossing circle $C$ corresponding to the vertex.  In $L_{B,0}$, at most one crossing can be associated to any crossing circle.  So the two crossings from Lemma \ref{lemma:tri-squares-assoc} must actually be the same crossing of the diagram.  Lemma \ref{lemma:distinct-crossings} implies that endpoints of $b$ and of $c$ map to distinct crossings, so those two cannot map to crossings associated to $C$.  Lemma \ref{lemma:ae-assoc} implies that if endpoints of $b$ and $d$ map to a crossing associated to $C$, then so does $a$, and again Lemma \ref{lemma:distinct-crossings} implies we have two crossings associated to $C$, contradicting the definition of $L_{B,0}$.  The only remaining possibility is that endpoints of $c$ and of $a$ map to a crossing associated to $C$.  But then by relabeling, we may again apply Lemma \ref{lemma:ae-assoc} to obtain a distinct crossing associated to $C$.  In all cases, we have a contradiction.
\end{proof}


\begin{lemma}\label{lemma:L2-no-5trisquares}
There cannot be five adjacent triangle--square pairs for the diagram of $L_{B,2}$.  
\end{lemma}

\begin{proof}
In three adjacent triangle--square pairs, there are four points where red edges meet blue edges to form triangles.  Lemmas \ref{lemma:tri-squares-assoc}, \ref{lemma:No-fg-assoc}, and \ref{lemma:ae-assoc} imply that three of these four points must map to crossings associated to the crossing circle corresponding to the blue vertex, and moreover, two of those four are adjacent to the top (or bottom by symmetry), and the last is adjacent to the bottom (resp.\ top).  Start with three such triangle--square pairs, and without loss of generality assume that the top two points are associated to the crossing circle.  This is shown on the left of Figure \ref{fig:5trisquare}.

\begin{figure}
  \includegraphics{5trisquare}
  \caption{Green circles correspond to points which map to crossings     associated with the crossing circle of the vertex.  Shown are     three, four, and five adjacent triangle--square pairs.  Note that     in the case of five, the squares shown in gray contradict Lemma~\ref{lemma:No-fg-assoc}.  }
  \label{fig:5trisquare}
\end{figure}

Now attempt to add a fourth adjacent triangle--square pair.  This new pair will form another set of three adjacent triangle--square pairs. It cannot be added to the top of the three, else the new set of three adjacent triangle--square pairs on the top will contradict Lemma~\ref{lemma:No-fg-assoc}.  Hence it must be added to the bottom, and the new point on the new triangle where blue meets red must be associated to the crossing circle of the blue vertex.  This is shown in the center of Figure~\ref{fig:5trisquare}.

Finally, attempt to add a fifth adjacent triangle--square pair.  This cannot be added to top or bottom, or we contradict Lemma \ref{lemma:No-fg-assoc}.  Thus there cannot be five adjacent triangle--square pairs.  
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{prop}\label{prop:L0-no-3adjbigons}
When $i=0$, the graph $\Gamma_B$ cannot contain three or more adjacent non-trivial bigons.
\end{prop}

\begin{proof}
Suppose the graph $\Gamma_B$ contains three adjacent non-trivial bigons.  By Lemma~\ref{lemma:no-blue-bigons}, these bigons cannot be disjoint from the red and green surfaces. The bigons cannot be disjoint from the red surface, for the following reason. The bigons would have to contain at least one green edge, by Lemma \ref{lemma:no-blue-bigons} (no non-trivial blue bigons). If there is a green edge which intersects the interior of a blue edge, this contradicts Lemma \ref{lemma:blue-green-bigons} (no blue-green bigons) or \ref{lemma:noBBG} (no blue-blue-green triangles). On the other hand, if both endpoints of the green edge are the same vertex of $\Gamma_B$, this contradicts Lemma \ref{lemma:NoGreenLoop} (no green monogons). If the endpoints of the green edge are distinct vertices of $\Gamma_B$, this implies that the edges of the blue bigons are trivial, which is contrary to hypothesis. So, the blue bigons intersect the red surface. Lemma~\ref{lemma:red-blue-bigons} (no red-blue bigons) implies any intersection with the red surface must run straight through all three adjacent bigons.  An outermost such intersection cuts off three adjacent blue--blue--red triangles.

By Lemma~\ref{lemma:adjacent-BBR-triples}, there cannot be a single such intersection of red, cutting off two pairs of three adjacent blue--blue--red triangles adjacent across the red edges.  Hence there are at least two such intersections of red, and the outermost two cut off three adjacent red triangles and three adjacent red squares.  But now Lemma~\ref{lemma:L0-no-3trisquares} implies that this is impossible when $i=0$.  
\end{proof}

\begin{prop}\label{prop:L2-no-5adjbigons}
When $i=2$, the graph $\Gamma_B$ cannot contain five or more adjacent non-trivial bigons.
\end{prop}

\begin{proof}
Suppose the graph contains five adjacent non-trivial bigons.  As in the proof of Proposition~\ref{prop:L0-no-3adjbigons}, we argue that the bigons cannot be disjoint green and red, by Lemma~\ref{lemma:no-blue-bigons}, cannot be disjoint red, by Lemmas~\ref{lemma:blue-green-bigons}, \ref{lemma:NoGreenLoop} and~\ref{lemma:noBBG}, and red intersections run through each bigon, splitting off triangles and squares by Lemma~\ref{lemma:red-blue-bigons}.  Again Lemma~\ref{lemma:adjacent-BBR-triples} implies there is more than one intersection of red, and the two outermost intersections cut off five adjacent triangles adjacent five adjacent squares across red edges. This contradicts Lemma~\ref{lemma:L2-no-5trisquares}.
\end{proof}

This completes the proof of Theorem \ref{thm:Bincompressible}.

